Sparse Logit Sampling: Accelerating Knowledge Distillation in LLMs

Knowledge distillation can be a cost-effective technique to distill knowledge in Large Language Models, if the teacher output logits can be pre-computed and cached. However, successfully applying this to pre-training remains largely unexplored. In this work, we prove that naive approaches for sparse knowledge distillation such as caching Top-K probabilities, while intuitive, provide biased estimates of teacher probability distribution to the student, resulting in suboptimal performance and calibration. We propose an importance-sampling-based method `Random Sampling Knowledge Distillation', which provides unbiased estimates, preserves the gradient in expectation, and requires storing significantly sparser logits. Our method enables faster training of student models with marginal overhead (<10%) compared to cross-entropy based training, while maintaining competitive performance compared to full distillation, across a range of model sizes from 300M to 3B.

==> tables/vanilla_topk_ce.tex <==
\begin{table}[H]
\begin{center}
\begin{adjustbox}{max width=0.9\linewidth}
\begin{tabular}{S[table-format=4]S[table-format=1.2, round-mode=places, round-precision=2]S[table-format=1.2, round-mode=places, round-precision=2]S[table-format=3\%, round-mode=places, round-precision=0]}
\toprule
    \textbf{Top-K} & \textbf{Orig LM} & \textbf{LM}  & \textbf{\% CE to}  \\
    \textbf{Tokens} & \textbf{Loss} & \textbf{Loss $\downarrow$}  & \textbf{FullKD $\uparrow$}  \\
    \midrule
    \text{CE} & 2.80668 & 2.80668 & 0\% \\
    \midrule
    50 &  2.80378  & 2.77174 & 50.07165377\% \\
    300  & 2.76044  & 2.74388 & 89.99713385\% \\
    5000 & \text{-} & 2.73948 & 96.30266552\% \\
    \midrule
    \text{FullKD} & 2.74698   & \bfseries 2.7369 & \bfseries 100\% \\
    \bottomrule
\end{tabular}
\label{table: Vanilla Top-k-CE}
\end{adjustbox}
\end{center}
\caption{Vanilla Top-k with $0.1$ CE Loss}
\end{table}
